From Charts to Code: A Hierarchical Benchmark for Multimodal Models

We introduce Chart2Code, a new benchmark for evaluating the chart understanding and code generation capabilities of large multimodal models (LMMs). Chart2Code is explicitly designed from a user-driven perspective, capturing diverse real-world scenarios and progressively increasing task difficulty. It consists of three levels: Level 1 (Chart Reproduction) reproduces charts from a reference figure and user query; Level 2 (Chart Editing) involves complex modifications such as changing chart types or adding elements; and Level 3 (Long-Table to Chart Generation) requires models to transform long, information-dense tables into faithful charts following user instructions. To our knowledge, this is the first hierarchical benchmark that reflects practical chart2code usage while systematically scaling task complexity. In total, Chart2Code contains 2,023 tasks across 22 chart types, paired with multi-level evaluation metrics that assess both code correctness and the visual fidelity of rendered charts. We benchmark 25 state-of-the-art (SoTA) LMMs, including both proprietary and the latest open-source models such as GPT-5, Qwen2.5-VL, InternVL3/3.5, MiMo-VL, and Seed-1.6-VL. Experimental results demonstrate that even the SoTA model GPT-5 averages only 0.57 on code-based evaluation and 0.22 on chart-quality assessment across the editing tasks, underscoring the difficulty of Chart2Code. We anticipate this benchmark will drive advances in multimodal reasoning and foster the development of more robust and general-purpose LMMs. Our code and data are available on Chart2Code.

==> figures/code_example/box_12_v4_old.tex <==
import pandas as pd
import matplotlib.pyplot as plt
import seaborn as sns
import matplotlib.gridspec as gridspec

data = {
    "TopK_65k_256": [-0.4625, -0.4049, -0.4268, -0.4401, -0.4844, 0.4156, 0.4058, 0.4866, 0.4601, 0.4708, 0.4021, 0.497, 0.4832, 0.4212, 0.4182, 0.5683, 0.5804, 0.6025, 0.5932, 0.5791, 0.6112, 0.5639, 0.5792, 0.5866, 0.5956, 0.7114, 0.688, 0.7006, 0.7037, 0.6819, 0.7043, 0.6868, 0.6826, 0.718, 0.7186, 0.7123, 0.6922, 0.6839, 0.7074, 0.6976, 0.8946, 0.9394, 0.8841, 0.9891, 0.9111, 0.9595, 0.9174, 0.9424, 0.9456, 0.9022, 0.9964, 0.973, 0.9927, 0.9874, 0.9517, 0.9906, 0.8906, 0.9035, 0.8854, 0.919],
    "MatryoshkaTopk_65k_256": [-0.0806, -0.0864, -0.0586, -0.0822, -0.086, 0.3043, 0.2641, 0.3302, 0.2575, 0.3487, 0.3272, 0.2699, 0.2506, 0.3315, 0.3207, 0.5958, 0.6043, 0.4648, 0.5217, 0.4732, 0.6226, 0.5747, 0.5162, 0.4627, 0.5122, 0.7325, 0.773, 0.7638, 0.7887, 0.7472, 0.712, 0.7713, 0.7761, 0.7561, 0.7771, 0.7494, 0.7523, 0.7428, 0.7025, 0.7108, 0.9031, 0.9636, 0.9314, 0.9509, 0.9908, 0.9249, 0.941, 0.9756, 0.9229, 0.9077, 0.929, 0.9161, 0.993, 0.9808, 0.9633, 0.9871, 0.9804, 0.9187, 0.9893, 0.9539],
    "GemmaScope_65k": [-0.0596, -0.0552, -0.0841, -0.0945, -0.0886, 0.3427, 0.3818, 0.3861, 0.3007, 0.3511, 0.3417, 0.3222, 0.312, 0.3338, 0.3943, 0.5646, 0.6038, 0.6406, 0.5727, 0.6944, 0.6925, 0.5504, 0.5994, 0.5602, 0.557, 0.8037, 0.861, 0.8503, 0.8051, 0.8279, 0.8908, 0.824, 0.8145, 0.8489, 0.8986, 0.8242, 0.8672, 0.8762, 0.8238, 0.8728, 0.9684, 0.9816, 0.9817, 0.9768, 0.9545, 0.9918, 0.966, 0.9593, 0.952, 0.9795, 0.9839, 0.9508, 0.9756, 0.9613, 0.9823, 0.9587, 0.9845, 0.9693, 0.9968, 0.9569],
    "Random_init_65k_256": [-0.2659, -0.2887, -0.2075, -0.2123, -0.2742, 0.266, 0.2817, 0.2555, 0.253, 0.2242, 0.2093, 0.2897, 0.29, 0.2633, 0.2339, 0.341, 0.3636, 0.3738, 0.3732, 0.3668, 0.3585, 0.325, 0.3297, 0.3739, 0.3564, 0.4509, 0.4601, 0.5164, 0.4505, 0.4661, 0.5049, 0.5192, 0.5152, 0.4724, 0.5212, 0.4737, 0.4825, 0.5246, 0.515, 0.5349, 0.9658, 0.9568, 0.9094, 0.9368, 0.9265, 0.9244, 0.9973, 0.9393, 0.9892, 0.9631, 0.9795, 0.9503, 0.9577, 0.9493, 0.9195, 0.9722, 0.9281, 0.9024, 0.9645, 0.9177],
}

clean_data = {k: [x for x in v if x is not None] for k, v in data.items()}
df = pd.DataFrame(clean_data).melt(var_name="SAE Type", value_name="Pearson Correlation")

sns.set_theme(style="whitegrid", rc={'grid.color': '#D3D3D3', 'axes.facecolor': 'white'})
fig = plt.figure(figsize=(14, 10))
gs = gridspec.GridSpec(2, 2, height_ratios=[2, 1])

ax_main = fig.add_subplot(gs[0, :])
ax_hist1 = fig.add_subplot(gs[1, 0])
ax_hist2 = fig.add_subplot(gs[1, 1])

fig.suptitle("Comprehensive Analysis of Pearson Correlation", fontsize=20, fontweight='bold')

# --- Top Plot: Raincloud Plot ---
order = ["TopK_65k_256", "MatryoshkaTopk_65k_256", "GemmaScope_65k", "Random_init_65k_256"]
colors = ["#FFC0A0", "#B0E0B0", "#B9A0E0", "#FFE4C4"]

# Half-violin
sns.violinplot(x="SAE Type", y="Pearson Correlation", data=df, order=order, ax=ax_main,
               inner=None, palette=colors, cut=0, hue="SAE Type", legend=False)
for collection in ax_main.collections:
    collection.set_alpha(0.7)

# Jittered points
sns.stripplot(x="SAE Type", y="Pearson Correlation", data=df, order=order, ax=ax_main,
              jitter=0.1, color='black', size=2.5, alpha=0.3)

# Boxplot
sns.boxplot(x="SAE Type", y="Pearson Correlation", data=df, order=order, ax=ax_main,
            width=0.2, fliersize=0,
            boxprops={'facecolor': 'none', 'edgecolor': 'black', 'linewidth': 1.5},
            whiskerprops={'color': 'black', 'linewidth': 1.2},
            capprops={'color': 'black', 'linewidth': 1.2},
            medianprops={'color': 'black', 'linewidth': 2})

ax_main.set_title("Overall Distribution (Raincloud Plot)", fontsize=16)
ax_main.set_xlabel("")
ax_main.set_ylabel("Pearson Correlation", fontsize=14)
ax_main.set_ylim(-0.5, 1.05)
ax_main.tick_params(axis='x', labelsize=12, labelrotation=-20)
ax_main.tick_params(axis='y', labelsize=12)

# --- Bottom-Left Plot: Histogram for GemmaScope ---
gemma_data = df[df["SAE Type"] == "GemmaScope_65k"]["Pearson Correlation"]
sns.histplot(gemma_data, ax=ax_hist1, bins=15, kde=True, color=colors[2], stat="density")
ax_hist1.set_title("Distribution of GemmaScope_65k", fontsize=14)
ax_hist1.set_xlabel("Pearson Correlation", fontsize=12)
ax_hist1.set_ylabel("Density", fontsize=12)
ax_hist1.axvline(gemma_data.mean(), color='red', linestyle='--', label=f'Mean: {gemma_data.mean():.2f}')
ax_hist1.legend()

# --- Bottom-Right Plot: Histogram for Random_init ---
random_data = df[df["SAE Type"] == "Random_init_65k_256"]["Pearson Correlation"]
sns.histplot(random_data, ax=ax_hist2, bins=15, kde=True, color=colors[3], stat="density")
ax_hist2.set_title("Distribution of Random_init_65k_256", fontsize=14)
ax_hist2.set_xlabel("Pearson Correlation", fontsize=12)
ax_hist2.set_ylabel("")
ax_hist2.axvline(random_data.mean(), color='red', linestyle='--', label=f'Mean: {random_data.mean():.2f}')
ax_hist2.legend()

sns.despine(fig=fig)
plt.tight_layout(rect=[0, 0, 1, 0.96])
plt.show()


==> figures/code_example/combination_16_v5_old.tex <==
import numpy as np
import matplotlib.pyplot as plt
import matplotlib.patches as mpatches
import matplotlib.gridspec as gridspec

np.random.seed(0)
runs = np.arange(5, 15)
mean35 = [2.5, 1.8, 1.6, 1.1, 1.0, 0.9, 0.5, 0.4, 0.2, 0.1]
std35  = [0.5, 0.4, 0.4, 0.3, 0.3, 0.3, 0.2, 0.2, 0.1, 0.1]
mean4  = [1.0, 0.7, 0.6, 0.4, 0.3, 0.4, 0.3, 0.1, 0.05, 0.02]
std4   = [0.2, 0.15,0.15,0.1, 0.1, 0.1, 0.1, 0.05,0.02,0.01]
data35 = [np.clip(np.random.normal(m, s, 100), 0, None) for m, s in zip(mean35, std35)]
data4  = [np.clip(np.random.normal(m, s, 100), 0, None) for m, s in zip(mean4, std4)]
tool_wear = np.array([0.15, 0.20, 0.25, 0.28, 0.27, 0.29, 0.38, 0.42, 0.45, 0.48])

# 1. 创建 GridSpec 布局
fig = plt.figure(figsize=(18, 10))
gs = gridspec.GridSpec(2, 2, width_ratios=[3, 2], height_ratios=[1, 1])
ax_main = fig.add_subplot(gs[:, 0])
ax_growth = fig.add_subplot(gs[0, 1])
ax_compare = fig.add_subplot(gs[1, 1])

# --- 2. 主图 (左侧) ---
pos1 = runs - 0.2
pos2 = runs + 0.2
# 转换为小提琴图
vp1 = ax_main.violinplot(data35, positions=pos1, widths=0.4, showmedians=True)
vp2 = ax_main.violinplot(data4, positions=pos2, widths=0.4, showmedians=True)
for pc in vp1['bodies']: pc.set_facecolor('#8dd3c7'); pc.set_edgecolor('black'); pc.set_alpha(0.7)
for pc in vp2['bodies']: pc.set_facecolor('#80b1d3'); pc.set_edgecolor('black'); pc.set_alpha(0.7)
for partname in ('cbars', 'cmins', 'cmaxes', 'cmedians'):
    vp1[partname].set_edgecolor('black')
    vp2[partname].set_edgecolor('black')

ax_main.set_xticks(runs)
ax_main.set_xlabel("Runs", fontsize=14)
ax_main.set_ylabel("RMSE Distribution", fontsize=14)
ax_main.tick_params(axis='both', labelsize=12)
ax_main.grid(True, linestyle="--", alpha=0.6)
ax_main.set_title("A) Model Performance Distribution vs. Tool Wear", fontsize=16, loc='left')

ax_wear = ax_main.twinx()
ax_wear.plot(runs, tool_wear, color="red", marker="o", markersize=6, linewidth=2)
ax_wear.set_ylabel("Tool Wear (mm)", color="red", fontsize=14)
ax_wear.tick_params(axis='y', labelsize=12, labelcolor="red")
patch1 = mpatches.Patch(color="#8dd3c7", label="GPT-3.5-Turbo")
patch2 = mpatches.Patch(color="#80b1d3", label="GPT-4")
line3  = plt.Line2D([], [], color="red", marker="o", label="Tool Wear")
ax_main.legend(handles=[patch1, patch2, line3], loc="upper right")

# --- 3. 右上图 (ax_growth) ---
wear_growth = (tool_wear[1:] - tool_wear[:-1]) / tool_wear[:-1] * 100
growth_runs = runs[1:]
colors = ['#d95f02'] * len(wear_growth)
max_growth_idx = np.argmax(wear_growth)
colors[max_growth_idx] = '#e31a1c' # 5. 高亮最大增长
bars = ax_growth.bar(growth_runs, wear_growth, color=colors)
ax_growth.set_title("B) Tool Wear Growth Rate", fontsize=16, loc='left')
ax_growth.set_xlabel("Run", fontsize=12)
ax_growth.set_ylabel("Growth Rate (%)", fontsize=12)
ax_growth.tick_params(axis='both', labelsize=10)
ax_growth.grid(axis='y', linestyle='--', alpha=0.6)

# --- 4. 右下图 (ax_compare) ---
median35 = [np.median(d) for d in data35]
median4 = [np.median(d) for d in data4]
# 5. 高亮与最大磨损增长对应的点
highlight_run_idx = max_growth_idx + 1 
ax_compare.scatter(median35, median4, c=runs, cmap='viridis', s=60, alpha=0.8)
ax_compare.scatter(median35[highlight_run_idx], median4[highlight_run_idx], 
                   facecolors='none', edgecolors='#e31a1c', s=200, linewidth=2.5,
                   label=f'Run {runs[highlight_run_idx]} (Max Wear Growth)')

lims = [min(ax_compare.get_xlim()[0], ax_compare.get_ylim()[0]),
        max(ax_compare.get_xlim()[1], ax_compare.get_ylim()[1])]
ax_compare.plot(lims, lims, 'k--', alpha=0.7, zorder=0, label='y = x (Equal Performance)')
ax_compare.set_title("C) Median RMSE: GPT-3.5 vs. GPT-4", fontsize=16, loc='left')
ax_compare.set_xlabel("GPT-3.5 Median RMSE", fontsize=12)
ax_compare.set_ylabel("GPT-4 Median RMSE", fontsize=12)
ax_compare.tick_params(axis='both', labelsize=10)
ax_compare.grid(True, linestyle='--', alpha=0.6)
ax_compare.set_aspect('equal', adjustable='box')
ax_compare.legend(loc='upper left', fontsize=10)
ax_compare.text(0.95, 0.05, 'GPT-4 Better', transform=ax_compare.transAxes,
                ha='right', va='bottom', fontsize=12, color='green', style='italic')

# --- 5. 联动注释 ---
max_growth_run = growth_runs[max_growth_idx]
ax_main.axvspan(max_growth_run - 0.5, max_growth_run + 0.5, color='#e31a1c', alpha=0.2, zorder=0)
ax_main.annotate('Max Wear Growth', xy=(max_growth_run, 4.0), xytext=(max_growth_run, 5.0),
                 arrowprops=dict(facecolor='#e31a1c', shrink=0.05, width=1.5, headwidth=8),
                 fontsize=12, color='#e31a1c', ha='center', bbox=dict(boxstyle="round,pad=0.3", fc="white", ec="#e31a1c", lw=1))

fig.suptitle("Comprehensive Analysis of LLM-based Digital Twin Performance", fontsize=20, y=0.98)
plt.tight_layout(rect=[0, 0, 1, 0.95])
plt.show()


==> figures/code_example/combination_1_v5_old.tex <==
import matplotlib.pyplot as plt
import matplotlib.gridspec as gridspec
from matplotlib.patches import Rectangle, ConnectionPatch
import numpy as np

layers = list(range(2, 30))
cca_top1 = [0.997, 0.997, 0.9968, 0.9967, 0.9969, 0.997, 0.998, 0.998, 0.997, 0.997, 0.996, 0.995, 0.9955, 0.995, 0.995, 0.995, 0.996, 0.996, 0.996, 0.996, 0.996, 0.996, 0.996, 0.995, 0.995, 0.995, 0.994, 0.994]
cca_top3 = [0.94, 0.92, 0.865, 0.89, 0.92, 0.985, 0.97, 0.97, 0.92, 0.915, 0.86, 0.885, 0.925, 0.96, 0.988, 0.99, 0.995, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0, 1.0]
cca_top10 = [0.855, 0.86, 0.87, 0.864, 0.885, 0.907, 0.9, 0.895, 0.875, 0.89, 0.915, 0.915, 0.933, 0.955, 0.965, 0.975, 0.978, 0.979, 0.985, 0.99, 0.992, 0.993, 0.994, 0.995, 0.996, 0.995, 0.996, 0.995]
cka = [0.968, 0.972, 0.968, 0.965, 0.97, 0.978, 0.976, 0.972, 0.969, 0.951, 0.945, 0.949, 0.96, 0.966, 0.97, 0.975, 0.98, 0.985, 0.99, 0.992, 0.993, 0.994, 0.995, 0.995, 0.995, 0.995, 0.995, 0.995]

# Create figure with constrained layout
fig = plt.figure(figsize=(15, 10), constrained_layout=True)
gs = gridspec.GridSpec(2, 2, width_ratios=[2, 1], height_ratios=[1, 1], figure=fig)

ax_main = fig.add_subplot(gs[0, 0])
ax_box = fig.add_subplot(gs[0, 1])
ax_zoom = fig.add_subplot(gs[1, :])
ax_main_twin = ax_main.twinx()

# --- Main Plot (Top-Left) ---
bar_width = 0.6
bars = ax_main_twin.bar(layers, cka, width=bar_width, color='#bbbbbb', label='CKA', alpha=0.7, zorder=1)
line1, = ax_main.plot(layers, cca_top1, color='#1f77b4', marker='o', markersize=5, lw=1.5, label='CCA:Top 1', zorder=3)
line2, = ax_main.plot(layers, cca_top3, color='#ff7f0e', marker='*', markersize=6, lw=1.5, label='CCA:Top 3', zorder=3)
line3, = ax_main.plot(layers, cca_top10, color='#2ca02c', marker='D', markersize=5, lw=1.5, label='CCA:Top 10', zorder=3)

ax_main.set_zorder(ax_main_twin.get_zorder() + 1)
ax_main.patch.set_visible(False)
ax_main.set_ylabel('Average CCA Value', fontsize=12)
ax_main_twin.set_ylabel(r'Average CKA similarity($\delta^5$)', fontsize=12)
ax_main.set_ylim(0.84, 1.002)
ax_main_twin.set_ylim(0.95, 1.00)
ax_main.grid(True, linestyle='--', linewidth=0.5, alpha=0.7, zorder=0)
ax_main.set_title('Overall Trend Analysis', fontsize=14, pad=15)
handles = [line1, line2, line3, bars]
labels = [h.get_label() for h in handles]
ax_main.legend(handles, labels, loc='lower center', ncol=4, fontsize=10, bbox_to_anchor=(0.5, -0.25))

# --- Box Plot (Top-Right) ---
data_for_boxplot = [cca_top1, cca_top3, cca_top10, cka]
box_labels = ['CCA:Top 1', 'CCA:Top 3', 'CCA:Top 10', 'CKA']

box = ax_box.boxplot(data_for_boxplot, patch_artist=True,
                    boxprops=dict(facecolor='#d3d3d3', color='black'),
                    medianprops=dict(color='red', linewidth=2))
ax_box.set_xticklabels(box_labels)
ax_box.set_title('Data Distribution', fontsize=14, pad=15)
ax_box.set_ylabel('Value', fontsize=12)
ax_box.tick_params(axis='x', rotation=30, labelsize=10)
ax_box.grid(True, axis='y', linestyle='--', linewidth=0.5, alpha=0.7)

# --- Zoomed Plot (Bottom) ---
zoom_range = (10, 20)
ax_zoom.plot(layers, cca_top1, color='#1f77b4', marker='o', markersize=6, lw=1.5)
ax_zoom.plot(layers, cca_top3, color='#ff7f0e', marker='*', markersize=8, lw=1.5)
ax_zoom.plot(layers, cca_top10, color='#2ca02c', marker='D', markersize=6, lw=1.5)
ax_zoom.set_xlim(zoom_range)
ax_zoom.set_ylim(0.85, 1.0)
ax_zoom.set_xlabel('Center Layer', fontsize=12)
ax_zoom.set_ylabel('CCA Value', fontsize=12)
ax_zoom.set_title(f'Zoomed View (Layers {zoom_range[0]}-{zoom_range[1]})', fontsize=14, pad=15)
ax_zoom.grid(True, linestyle='--', linewidth=0.5, alpha=0.7)

# --- Visual Connection ---
rect = Rectangle((zoom_range[0], 0.84), zoom_range[1] - zoom_range[0], 1.002 - 0.84,
                 facecolor='grey', alpha=0.2, edgecolor='red', linestyle='--')
ax_main.add_patch(rect)

# Create connection lines
con1 = ConnectionPatch(xyA=(zoom_range[0], 0.84), xyB=(zoom_range[0], 1.0),
                       coordsA=ax_main.transData, coordsB=ax_zoom.transData,
                       color='red', linestyle='--', lw=1)
con2 = ConnectionPatch(xyA=(zoom_range[1], 0.84), xyB=(zoom_range[1], 1.0),
                       coordsA=ax_main.transData, coordsB=ax_zoom.transData,
                       color='red', linestyle='--', lw=1)
fig.add_artist(con1)
fig.add_artist(con2)

# Remove tight_layout and let constrained_layout handle it
plt.show()

==> figures/code_example/combination_27_v5_old.tex <==
import numpy as np
import matplotlib.pyplot as plt
import matplotlib.gridspec as gridspec

years = np.array([2017, 2018, 2019, 2020, 2021, 2022, 2023, 2024])
x = np.arange(len(years))
y = np.array([39, 68, 152, 189, 285, 367, 408, 654])

# 1. 数据操作
cumulative_y = np.cumsum(y) # 累计总和
last_3_years_data = y[-3:]
last_3_years_labels = years[-3:]

# 3. 布局修改：使用GridSpec创建复杂布局
fig = plt.figure(figsize=(16, 9))
gs = gridspec.GridSpec(2, 3, figure=fig)

ax1 = fig.add_subplot(gs[:, 0:2]) # 主图
ax2 = fig.add_subplot(gs[0, 2])  # 右上副图
ax3 = fig.add_subplot(gs[1, 2])  # 右下副图

fig.suptitle('Comprehensive Analysis of Research Growth (2017-2024)', fontsize=22, fontweight='bold')

# --- 主图 (ax1): 年度数量与趋势 ---
ax1.bar(x, y, color='#1a5276', width=0.5, label='Annual Studies')
y_exp = 35.665 * np.exp(0.378 * x)
ax1.plot(x, y_exp, linestyle=':', color='red', linewidth=2, label='Exponential Trend')
for i, val in enumerate(y):
    ax1.text(i, val + 10, str(val), ha='center', va='bottom', color='gray')
ax1.set_title('Annual Number of Studies and Trend', fontsize=16, pad=10)
ax1.set_xlabel('Year', fontsize=14, color='grey')
ax1.set_ylabel('Number of Studies', fontsize=14, color='grey')
ax1.set_xticks(x)
ax1.set_xticklabels(years, fontsize=12, color='grey')
ax1.set_ylim(0, 750)
ax1.legend(loc='upper left')
for spine in ['top', 'right', 'left']:
    ax1.spines[spine].set_visible(False)
ax1.spines['bottom'].set_color('grey')

# --- 右上副图 (ax2): 累计增长面积图 ---
# 2. 图表类型转换与组合
ax2.fill_between(years, cumulative_y, color='#5dade2', alpha=0.6)
ax2.plot(years, cumulative_y, color='#1a5276', marker='o')
ax2.set_title('Cumulative Growth', fontsize=16, pad=10)
ax2.set_xlabel('Year', fontsize=12, color='grey')
ax2.set_ylabel('Total Studies', fontsize=12, color='grey')
for spine in ['top', 'right']:
    ax2.spines[spine].set_visible(False)
ax2.grid(axis='y', linestyle='--', alpha=0.7)
ax2.text(years[-1], cumulative_y[-1], f' Total:\n {cumulative_y[-1]}', ha='right', va='top', fontsize=12, fontweight='bold')


# --- 右下副图 (ax3): 近三年贡献甜甜圈图 ---
# 2. 图表类型转换与组合
colors = ['#1abc9c', '#f1c40f', '#e74c3c']
wedges, texts, autotexts = ax3.pie(last_3_years_data,
                                   labels=last_3_years_labels,
                                   autopct='%1.1f%%',
                                   startangle=90,
                                   colors=colors,
                                   pctdistance=0.85,
                                   textprops={'fontsize': 12, 'fontweight':'bold'})
# 4. 属性调整与注释：创建甜甜圈效果
centre_circle = plt.Circle((0, 0), 0.70, fc='white')
ax3.add_artist(centre_circle)
ax3.set_title('Contribution in Last 3 Years', fontsize=16, pad=10)
ax3.text(0, 0, f'Total:\n{sum(last_3_years_data)}', ha='center', va='center', fontsize=14, fontweight='bold')
plt.setp(autotexts, size=8, weight="bold", color="white")

plt.tight_layout(rect=[0, 0, 1, 0.95])
plt.show()


==> figures/code_example/combination_67_old.tex <==
# == CB_38 figure code ==
import matplotlib.pyplot as plt
import numpy as np
import matplotlib.colors as mcolors

# == CB_38 figure data ==
capabilities = {
    'Basic Knowledge': [
        'Vocabulary', 'Syntax', 'Semantics', 'Discourse', 'Logic', 'Math Reasoning'
    ],
    'Domain Knowledge': [
        'History', 'Politics', 'Science', 'Technology',
        'Arts', 'Economics', 'Medicine'
    ],
    'Dialect Comprehension': [
        'Chitchat', 'Slang', 'Accent', 'Colloquialisms'
    ],
    'Paralinguistic & Implicit Semantics': [
        'Emotion Perception', 'User Intent', 'Humor Detection', 'Sarcasm Detection'
    ],
    'Safety & Values': [
        'Toxicity Detection', 'Bias Detection', 'Privacy Protection', 'Fairness'
    ],
    'Scene': [
        'Age Response', 'Concern Recognition', 'NSV Handling'
    ],
    'System Abilities': [
        'Noise-zh', 'Age-zh', 'ParaMix-zh'
    ]
}

datasets = {
    'Basic Knowledge': [
        'LlamaQA-en', 'LlamaQA-zh',
        'TriviaQA-en', 'TriviaQA-zh',
        'WebQA-en',    'WebQA-zh'
    ],
    'Domain Knowledge': [
        'Cival-zh', 'ChineseQA-catch',
        'ChineseQA-gsm', 'ChineseQA-car',
        'ChineseQA-other'
    ],
    'Dialect Comprehension': [
        'Chitchat', 'User Dialogue', 'Dialect Chat'
    ],
    'Paralinguistic & Implicit Semantics': [
        'ESD-zh', 'AED-zh', 'Age-zh'
    ],
    'Safety & Values': [
        'Toxicity-zh', 'Bias-zh', 'Hate-zh'
    ],
    'Scene': [
        'CustomerSupport', 'LegalDoc', 'SocialMedia'
    ],
    'Acoustic Robustness': [
        'Noise-zh', 'ParaMix-zh'
    ]
}

def lighten_color(color, amount=0.5):
    rgb = mcolors.to_rgb(color)
    return tuple(rgb[i] + (1.0 - rgb[i]) * amount for i in range(3))

def prepare_sunburst(groups):
    inner_labels = list(groups.keys())
    inner_sizes  = [len(groups[k]) for k in inner_labels]
    cmap = plt.get_cmap('tab20')
    inner_colors = [cmap(i*2) for i in range(len(inner_labels))]
    outer_labels = []
    outer_sizes  = []
    outer_colors = []
    for i, key in enumerate(inner_labels):
        for sub in groups[key]:
            outer_labels.append(sub)
            outer_sizes.append(1)
            outer_colors.append(lighten_color(inner_colors[i], 0.6))
    return inner_labels, inner_sizes, inner_colors, outer_labels, outer_sizes, outer_colors

inner_a, size_a, col_a, outer_a, osize_a, ocol_a = prepare_sunburst(capabilities)
inner_b, size_b, col_b, outer_b, osize_b, ocol_b = prepare_sunburst(datasets)

categories = [
    'Basic Knowledge', 'Dialect Comprehension', 'Chitchat',
    'Emotion P&R',   'Age P&R',               'NSV P&R',
    'Scene',         'Acoustic Robustness',   'CER',
    'DNSMOS'
]
ranges = {
    'Basic Knowledge':        (8.96, 32.93),
    'Dialect Comprehension':  (0.00, 54.10),
    'Chitchat':               (9.21, 80.89),
    'Emotion P&R':            (8.32, 53.17),
    'Age P&R':                (3.63, 42.53),
    'NSV P&R':                (0.77, 9.19),
    'Scene':                  (0.19, 37.11),
    'Acoustic Robustness':    (10.70, 45.30),
    'CER':                    (1.69, 17.27),
    'DNSMOS':                 (2.46, 3.52)
}
models = {
    'GLM-4-Voice':        [12.0,  20.0,  30.0, 25.0, 15.0,  3.0, 10.0, 20.0, 10.0, 2.60],
    'MiniCMP@PMIx-2.6':   [10.0,  18.0,  25.0, 20.0, 12.0,  2.0,  8.0, 18.0, 12.0, 2.50],
    'BaiChuan-1.5':       [14.0,  22.0,  35.0, 30.0, 18.0,  4.0, 12.0, 22.0,  8.0, 2.80],
    'LLaMA-3-Omni':       [15.0,  25.0,  40.0, 35.0, 20.0,  5.0, 15.0, 25.0,  7.0, 3.00],
    'SpeechGPT-2-prev':   [13.0,  21.0,  32.0, 28.0, 17.0,  3.5, 11.0, 21.0,  9.0, 2.70],
    'Freezec-Omni':       [16.0,  28.0,  50.0, 40.0, 25.0,  6.0, 18.0, 30.0,  6.0, 3.20],
    'Qwen2.5-Omni':       [17.0,  30.0,  60.0, 45.0, 28.0,  7.0, 20.0, 35.0,  5.0, 3.40],
    'Gemini-Audio':       [18.0,  32.0,  70.0, 50.0, 30.0,  8.0, 22.0, 40.0,  4.0, 3.50],
    'GPT4-Audio (24-12-17)': [20.0, 40.0,  80.0, 53.0, 42.0,  9.0, 37.0, 45.0,  2.0, 3.52]
}
model_stats = {}
for name, vals in models.items():
    normed = []
    for cat, v in zip(categories, vals):
        lo, hi = ranges[cat]
        if cat == 'CER':
            normed.append((hi - v) / (hi - lo))
        else:
            normed.append((v - lo) / (hi - lo))
    model_stats[name] = normed


# == figure plot ==
fig = plt.figure(figsize=(18.0, 6.0))
plt.subplots_adjust(left=0.05, right=0.85, wspace=0.7)

# -- (a) Evaluation capabilities sunburst --
ax1 = fig.add_subplot(1, 3, 1)

ax1.pie(
    osize_a, radius=1.2,
    labels=outer_a, rotatelabels=True, startangle=90,
    labeldistance=1.05,
    colors=ocol_a,
    wedgeprops=dict(width=0.3, edgecolor='white'),
    textprops=dict(fontsize=7)
)

wedges1, _ = ax1.pie(
    size_a, radius=0.8,
    labels=None, startangle=90,
    colors=col_a,
    wedgeprops=dict(width=0.3, edgecolor='white')
)
centre = plt.Circle((0, 0), 0.5, color='lightgray', linewidth=0)
ax1.add_artist(centre)
ax1.text(0, 0, 'Explicit\nSemantics',
         ha='center', va='center', fontsize=10, weight='bold')
ax1.set(aspect='equal')
ax1.set_title('(a) Evaluation capabilities', fontsize=12, pad=45)
ax1.legend(
    wedges1, inner_a,
    title='Capabilities',
    loc='center left',
    bbox_to_anchor=(1.3, 0.5),
    fontsize=9,
    frameon=False
)

# -- (b) Evaluation datasets sunburst --
ax2 = fig.add_subplot(1, 3, 2)
ax2.pie(
    osize_b, radius=1.2,
    labels=outer_b, rotatelabels=True, startangle=90,
    labeldistance=1.05,
    colors=ocol_b,
    wedgeprops=dict(width=0.3, edgecolor='white'),
    textprops=dict(fontsize=7)
)
wedges2, _ = ax2.pie(
    size_b, radius=0.8,
    labels=None, startangle=90,
    colors=col_b,
    wedgeprops=dict(width=0.3, edgecolor='white')
)
centre2 = plt.Circle((0, 0), 0.5, color='lightgray', linewidth=0)
ax2.add_artist(centre2)
ax2.text(0, 0, 'Explicit\nSemantics',
         ha='center', va='center', fontsize=10, weight='bold')
ax2.set(aspect='equal')
ax2.set_title('(b) Evaluation datasets', fontsize=12, pad=45)
ax2.legend(
    wedges2, inner_b,
    title='Datasets',
    loc='center left',
    bbox_to_anchor=(1.3, 0.5),
    fontsize=9,
    frameon=False
)

# -- (c) Overview of evaluation results (radar) --
ax3 = fig.add_subplot(1, 3, 3, projection='polar')

N = len(categories)
angles = np.linspace(0, 2*np.pi, N, endpoint=False).tolist()
angles += angles[:1]

ax3.set_theta_offset(np.pi/2)
ax3.set_theta_direction(-1)

ax3.xaxis.set_ticks(angles[:-1])
ax3.set_xticklabels([])     
ax3.grid(True, linestyle=':')

ax3.set_yticks([0.2, 0.4, 0.6, 0.8, 1.0])
ax3.set_ylim(0, 1)

for name, stat in model_stats.items():
    vals = stat + stat[:1]
    ax3.plot(angles, vals, label=name, linewidth=1.0)
    ax3.fill(angles, vals, alpha=0.05)

radar_labels = [
    'Basic\nKnowledge\n(8.96–32.93)',
    'Dialect\nComprehension\n(0.00–54.10)',
    'Chitchat\n(9.21–80.89)',
    'Emotion\nP&R\n(8.32–53.17)',
    'Age\nP&R\n(3.63–42.53)',
    'NSV\nP&R\n(0.77–9.19)',
    'Scene\n(0.19–37.11)',
    'Acoustic\nRobustness\n(10.70–45.30)',
    'CER\n(1.69–17.27)',
    'DNSMOS\n(2.46–3.52)'
]
for angle, label in zip(angles[:-1], radar_labels):
    ax3.text(
        angle, 1.35,       
        label,
        fontsize=7,
        ha='center',
        va='center'
    )

ax3.set_title('(c) Overview of evaluation results', fontsize=12, pad=45)
ax3.legend(
    loc='lower center',
    bbox_to_anchor=(0.5, -0.5),
    ncol=3,
    fontsize=7,
    frameon=False
)

plt.subplots_adjust(bottom=0.2)

plt.tight_layout()
plt.savefig("./datasets/CB_38.png")
plt.show()

==> figures/code_example/line_19_v5_old.tex <==
# == line_19 figure code ==
import matplotlib.pyplot as plt
import numpy as np
import matplotlib.gridspec as gridspec

# == line_19 figure data ==
epochs = np.arange(1, 31)

# FinTabNet variants
ftn_a1 = np.array([
    0.24, 0.29, 0.32, 0.33, 0.38, 0.39, 0.38, 0.41, 0.40, 0.42,
    0.41, 0.37, 0.42, 0.41, 0.42, 0.40, 0.41, 0.42, 0.39, 0.41,
    0.40, 0.42, 0.41, 0.43, 0.41, 0.42, 0.42, 0.43, 0.43, 0.44
])
ftn_a2 = np.array([
    0.21, 0.23, 0.25, 0.29, 0.30, 0.37, 0.37, 0.38, 0.40, 0.40,
    0.42, 0.41, 0.43, 0.42, 0.41, 0.42, 0.42, 0.41, 0.42, 0.43,
    0.41, 0.43, 0.42, 0.43, 0.42, 0.44, 0.43, 0.44, 0.44, 0.44
])
ftn_a3 = np.array([
    0.22, 0.29, 0.33, 0.38, 0.40, 0.38, 0.38, 0.42, 0.41, 0.43,
    0.42, 0.44, 0.41, 0.42, 0.43, 0.44, 0.42, 0.43, 0.41, 0.44,
    0.43, 0.44, 0.43, 0.44, 0.43, 0.44, 0.44, 0.44, 0.44, 0.44
])
ftn_a4 = np.array([
    0.24, 0.34, 0.32, 0.45, 0.47, 0.48, 0.51, 0.49, 0.53, 0.50,
    0.57, 0.56, 0.53, 0.57, 0.58, 0.53, 0.55, 0.57, 0.58, 0.53,
    0.55, 0.56, 0.54, 0.59, 0.57, 0.60, 0.61, 0.62, 0.59, 0.62
])
ftn_a5 = np.array([
    0.24, 0.32, 0.35, 0.42, 0.48, 0.64, 0.70, 0.66, 0.65, 0.69,
    0.68, 0.69, 0.71, 0.70, 0.71, 0.70, 0.76, 0.75, 0.75, 0.76,
    0.76, 0.77, 0.76, 0.77, 0.78, 0.76, 0.78, 0.76, 0.78, 0.75
])
ftn_a6 = np.array([
    0.35, 0.40, 0.48, 0.49, 0.49, 0.51, 0.60, 0.58, 0.60, 0.58,
    0.57, 0.59, 0.57, 0.58, 0.63, 0.63, 0.61, 0.62, 0.62, 0.61,
    0.64, 0.62, 0.63, 0.61, 0.63, 0.60, 0.62, 0.63, 0.59, 0.59
])

# PubTables‐1M baseline
pubtables = np.array([
    0.24, 0.43, 0.48, 0.55, 0.57, 0.64, 0.70, 0.66, 0.65, 0.69,
    0.68, 0.69, 0.71, 0.70, 0.71, 0.70, 0.76, 0.75, 0.75, 0.76,
    0.76, 0.77, 0.77, 0.78, 0.79, 0.78, 0.78, 0.78, 0.78, 0.75
])

# PT1M + FTN variants
pt1m_av1 = np.array([
    0.24, 0.43, 0.48, 0.49, 0.52, 0.61, 0.66, 0.65, 0.66, 0.68,
    0.69, 0.70, 0.69, 0.71, 0.70, 0.70, 0.75, 0.74, 0.74, 0.73,
    0.75, 0.74, 0.76, 0.74, 0.74, 0.74, 0.75, 0.75, 0.79, 0.78
])
pt1m_av6 = np.array([
    0.24, 0.45, 0.56, 0.62, 0.63, 0.67, 0.71, 0.76, 0.74, 0.77,
    0.75, 0.78, 0.77, 0.79, 0.80, 0.79, 0.76, 0.78, 0.79, 0.80,
    0.79, 0.80, 0.81, 0.82, 0.83, 0.82, 0.83, 0.82, 0.79, 0.78
])

# == Data Processing for Dashboard ==
# 1. Group data
fintabnet_group_data = np.array([ftn_a1, ftn_a2, ftn_a3, ftn_a4, ftn_a5, ftn_a6])
pt1m_based_group_data = np.array([pubtables, pt1m_av1, pt1m_av6])
all_models_data = np.vstack([fintabnet_group_data, pt1m_based_group_data])
all_models_labels = ['FTN.a1', 'FTN.a2', 'FTN.a3', 'FTN.a4', 'FTN.a5', 'FTN.a6', 'PubTables', 'PT1M+FTN.av1', 'PT1M+FTN.av6']

# 2. Calculate group stats
ftn_mean = np.mean(fintabnet_group_data, axis=0)
ftn_std = np.std(fintabnet_group_data, axis=0)
pt1m_mean = np.mean(pt1m_based_group_data, axis=0)
pt1m_std = np.std(pt1m_based_group_data, axis=0)

# 3. Final performance data
final_acc = all_models_data[:, -1]
sorted_indices = np.argsort(final_acc)
sorted_labels = [all_models_labels[i] for i in sorted_indices]
sorted_acc = final_acc[sorted_indices]
colors = ['tab:blue'] * 6 + ['tab:red'] * 3
sorted_colors = [colors[i] for i in sorted_indices]

# 4. Significant surpass point
diff = pt1m_av6 - pubtables
surpass_margin = 0.05
surpass_epoch_idx = np.where(diff > surpass_margin)[0]
first_surpass_epoch = epochs[surpass_epoch_idx[0]] if len(surpass_epoch_idx) > 0 else None

# 5. Performance vs. Stability data
mean_acc_all = np.mean(all_models_data, axis=1)
std_acc_all = np.std(all_models_data, axis=1)

# == Figure Plot ==
fig = plt.figure(figsize=(16, 12))
gs = gridspec.GridSpec(2, 2, figure=fig, hspace=0.4, wspace=0.3)
ax1 = fig.add_subplot(gs[0, 0])
ax2 = fig.add_subplot(gs[0, 1])
ax3 = fig.add_subplot(gs[1, 0])
ax4 = fig.add_subplot(gs[1, 1])
fig.suptitle('Comprehensive Model Performance Dashboard', fontsize=20)

# Plot 1: Group Performance Trends
ax1.plot(epochs, ftn_mean, color='tab:blue', label='FinTabNet Group (Mean)')
ax1.fill_between(epochs, ftn_mean - ftn_std, ftn_mean + ftn_std, color='tab:blue', alpha=0.2)
ax1.plot(epochs, pt1m_mean, color='tab:red', label='PT1M-based Group (Mean)')
ax1.fill_between(epochs, pt1m_mean - pt1m_std, pt1m_mean + pt1m_std, color='tab:red', alpha=0.2)
ax1.set_title('1. Performance Trend by Group')
ax1.set_xlabel('Epoch'); ax1.set_ylabel('Mean Acc$_{Con}$')
ax1.legend(); ax1.grid(True, alpha=0.3)

# Plot 2: Final Performance Ranking
ax2.barh(range(len(sorted_acc)), sorted_acc, color=sorted_colors)
ax2.set_yticks(range(len(sorted_labels)))
ax2.set_yticklabels(sorted_labels)
ax2.set_title('2. Final Accuracy Ranking (Epoch 30)')
ax2.set_xlabel('Final Acc$_{Con}$'); ax2.set_ylabel('Model')
ax2.grid(True, axis='x', alpha=0.3)
for index, value in enumerate(sorted_acc):
    ax2.text(value, index, f' {value:.3f}', va='center')

# Plot 3: Key Model Showdown
ax3.plot(epochs, pubtables, label='PubTables-1M (Baseline)', color='cyan')
ax3.plot(epochs, pt1m_av6, label='PT1M + FTN.av6 (Best)', color='peru')
if first_surpass_epoch:
    ax3.axvspan(first_surpass_epoch, epochs[-1], color='green', alpha=0.15, label=f'Significant Lead (>{surpass_margin})')
    ax3.annotate(f'Surpass at Epoch {int(first_surpass_epoch)}', 
                 xy=(first_surpass_epoch, pt1m_av6[int(first_surpass_epoch)-1]),
                 xytext=(15, 0.6),
                 arrowprops=dict(facecolor='black', arrowstyle='->'),
                 ha='center')
ax3.set_title('3. Key Model Duel')
ax3.set_xlabel('Epoch'); ax3.set_ylabel('Acc$_{Con}$')
ax3.legend(); ax3.grid(True, alpha=0.3)

# Plot 4: Performance vs. Stability
ax4.scatter(mean_acc_all, std_acc_all, c=colors, s=50, alpha=0.7)
ax4.set_title('4. Performance vs. Stability')
ax4.set_xlabel('Mean Accuracy (Performance)'); ax4.set_ylabel('Std. Dev. of Accuracy (Instability)')
ax4.grid(True, alpha=0.3)
# Annotate key points
best_model_idx = np.argmax(mean_acc_all)
most_stable_idx = np.argmin(std_acc_all)
least_stable_idx = np.argmax(std_acc_all)
for i in {best_model_idx, most_stable_idx, least_stable_idx}:
    ax4.text(mean_acc_all[i]+0.002, std_acc_all[i], all_models_labels[i], fontsize=9)

plt.tight_layout(rect=[0, 0.03, 1, 0.95])
# plt.savefig("./datasets/line_19.png")
plt.show()


==> figures/code_example/radar_40_old.tex <==
import numpy as np
import matplotlib.pyplot as plt

hours = np.arange(24)
angles = 2 * np.pi * hours / 24

no2 = np.array([128,114,102,83,86,120,118,126,108,127,115,107,
                115,109,113,125,123,130,123,143,120,131,122,104])

stationary = np.array([0.35,0.05,-0.02,-0.08,0.10,0.15,0.20,0.18,
                       0.22,0.40,0.50,0.25,0.10,0.05,-0.05,-0.10,
                       0.20,0.30,0.15,0.20,0.25,0.18,0.12,0.30])
bus_counts = np.array([0.10,0.02,-0.01,-0.05,0.12,0.18,0.15,0.20,
                       0.18,0.30,0.28,0.10,0.05,0.00,-0.02,-0.08,
                       0.10,0.25,0.12,0.15,0.18,0.16,0.10,0.22])
truck_counts = np.array([0.05,0.01,-0.02,-0.04,0.15,0.20,0.22,0.25,
                         0.20,0.30,0.22,0.12,0.04,0.02,-0.01,-0.06,
                         0.10,0.20,0.18,0.22,0.15,0.12,0.08,0.18])
industry_proximity = np.array([0.20,0.04,-0.03,-0.07,0.11,0.25,0.30,0.22,
                               0.28,0.35,0.28,0.18,0.08,0.05,-0.03,-0.05,
                               0.15,0.28,0.20,0.26,0.30,0.22,0.15,0.33])

fig = plt.figure(figsize=(10,10))
ax = fig.add_subplot(111, polar=True)
ax.set_theta_zero_location('N')
ax.set_theta_direction(-1)
ax.set_ylim(0,160)
ax.set_yticks([])
ax.set_xticks(angles)
ax.set_xticklabels([f'{h}:00' for h in hours], fontsize=12, fontweight='bold')

for th in angles:
    ax.plot([th, th], [0, 160], color='grey', linewidth=0.5)

baseline = 100
theta = np.linspace(0, 2*np.pi, 360)
ax.plot(theta, np.full_like(theta, baseline), linestyle='--', color='black', linewidth=1)
inner_circle = np.mean(no2)
ax.plot(theta, np.full_like(theta, inner_circle), linestyle='--', color='grey', linewidth=1)

ax.text(0, 0, r'NO$_2$Clock', fontsize=18, fontweight='bold', ha='center', va='center')

bar_width = 2*np.pi/24 * 0.2
offsets = np.array([-1.5, -0.5, 0.5, 1.5]) * bar_width
for vals, off, color, label in zip(
        [stationary, bus_counts, truck_counts, industry_proximity],
        offsets,
        ['tab:blue','tab:red','lightpink','skyblue'],
        ['β Stationary cars','β bus_counts','β truck_counts','β industry_proximity']):
    ax.bar(angles + off, vals * 100, bottom=baseline, width=bar_width, color=color, label=label)

scale = 0.8
no2_scaled = baseline + (no2 - baseline) * scale
ln, = ax.plot(angles, no2_scaled, color='black', linewidth=2, label='NO2 max value')
ax.fill(angles, no2_scaled, color='grey', alpha=0.7)

for ang, orig_val, r in zip(angles, no2, no2_scaled):
    ax.text(ang, r + 2, f'{orig_val}', ha='center', va='bottom', fontsize=8, color='black')

ax.text(np.deg2rad(30), baseline+15, '+ve', fontsize=14, fontweight='bold', ha='center')
ax.text(np.deg2rad(30), baseline-15, '-ve', fontsize=14, fontweight='bold', ha='center')

ax.legend(loc='upper right', bbox_to_anchor=(1.1,1.1), fontsize=10)

plt.show()

==> figures/code_example/radar_45_old.tex <==
import matplotlib.pyplot as plt
import numpy as np

# == New radar figure data ==

labels = ['Compute', 'Storage', 'Networking', 'Database', 'AI/ML', 'Security']
num_metrics = len(labels)
# angle of each axis in the plot (in radians)
angles = np.linspace(0, 2 * np.pi, num_metrics, endpoint=False).tolist()
# complete the loop
angles += angles[:1]

# Values for each industry's cloud service adoption (0-100 scale)
data = {
    'Tech Startup': [85, 60, 70, 80, 90, 75],
    'Financial Services': [70, 65, 60, 85, 50, 95],
    'Healthcare': [60, 90, 55, 75, 65, 85],
    'Retail': [80, 70, 65, 80, 75, 70],
    'Manufacturing': [75, 60, 80, 70, 55, 80],
    'Education': [70, 85, 50, 65, 45, 70],
    'Government': [65, 80, 60, 70, 40, 90],
    'Media': [80, 95, 75, 70, 60, 70],
    'Logistics': [75, 65, 85, 80, 50, 75],
    'Energy': [70, 60, 80, 70, 55, 85],
}

industries = list(data.keys())

# New modern color scheme
colors = [
    '#4CAF50',  # Green
    '#2196F3',  # Blue
    '#FFC107',  # Amber
    '#E91E63',  # Pink
    '#9C27B0',  # Purple
    '#00BCD4',  # Cyan
    '#FF5722',  # Deep Orange
    '#795548',  # Brown
    '#607D8B',  # Blue Grey
    '#CDDC39'   # Lime
]

# == figure plot ==

fig, axes = plt.subplots(2, 5,
                         figsize=(15.0, 9.0), # Slightly larger for readability
                         subplot_kw=dict(polar=True))
axes = axes.ravel()

for ax, name in zip(axes, industries):
    vals = data[name]
    # close the loop
    vals_loop = vals + vals[:1]
    i = industries.index(name) % len(colors)  # cycle through colors
    # plot the radar chart
    ax.plot(angles, vals_loop, color=colors[i], linewidth=2)
    ax.fill(angles, vals_loop, color=colors[i], alpha=0.25)
    # set the labels for each axis
    ax.set_xticks(angles[:-1])
    ax.set_xticklabels(labels, fontsize=10)
    
    # radial ticks and limits
    max_val = max(vals)
    # build six evenly spaced ticks from 0 to max_val
    rticks = np.linspace(0, max_val, 6)
    ax.set_yticks(rticks)
    ax.set_yticklabels([f"{int(x)}" for x in rticks], fontsize=8)
    ax.set_ylim(0, max_val * 1.1) # Add a small buffer to max_val
    
    # title
    ax.set_title(name, fontsize=12, fontweight='bold', pad=10)
    
    # light grid
    ax.grid(color='gray', linestyle='--', linewidth=0.5, alpha=0.7)
    ax.spines['polar'].set_linewidth(1.0)

    # add the legend‐style box in a suitable subplot (e.g., Healthcare)
    if name == 'Healthcare':
        legend_txt = (
            "Compute   - Virtual Machines, Containers\n"
            "Storage   - Object, Block, File Storage\n"
            "Networking- VPC, Load Balancers, CDN\n"
            "Database  - SQL, NoSQL, Data Warehouses\n"
            "AI/ML     - Machine Learning Services\n"
            "Security  - IAM, Encryption, WAF"
        )
        ax.text(0.5, -0.3, legend_txt,
                transform=ax.transAxes,
                fontsize=8,
                verticalalignment='top',
                bbox=dict(boxstyle='round', facecolor='none',
                          edgecolor='gray', linestyle='--'))

plt.tight_layout(rect=[0, 0, 1, 0.96]) # Adjust layout to make space for a potential suptitle
plt.suptitle('Cloud Service Adoption Across Industries', fontsize=16, fontweight='bold', y=0.99)
plt.savefig("./datasets_level2/radar_15.png", bbox_inches="tight", dpi=300)  # Save the figure
plt.show()

==> figures/code_example/table_60_instruction_3_request_modified_old.tex <==
import numpy as np
import matplotlib.pyplot as plt

# Data
dates = [
    "2020-01-01","2020-02-01","2020-03-01","2020-04-01","2020-05-01","2020-06-01",
    "2020-07-01","2020-08-01","2020-09-01","2020-10-01","2020-11-01","2020-12-01",
    "2021-01-01","2021-02-01","2021-03-01","2021-04-01","2021-05-01","2021-06-01",
    "2021-07-01","2021-08-01","2021-09-01","2021-10-01","2021-11-01","2021-12-01",
    "2022-01-01","2022-02-01","2022-03-01","2022-04-01","2022-05-01","2022-06-01",
    "2022-07-01","2022-08-01","2022-09-01","2022-10-01","2022-11-01","2022-12-01",
    "2023-01-01","2023-02-01","2023-03-01","2023-04-01","2023-05-01","2023-06-01",
    "2023-07-01","2023-08-01","2023-09-01","2023-10-01","2023-11-01","2023-12-01",
    "2024-01-01","2024-02-01","2024-03-01","2024-04-01","2024-05-01","2024-06-01",
    "2024-07-01","2024-08-01","2024-09-01"
]
commodities = ["Energy", "Metals", "Food"]
values = [
    [4.7, -13.5, -46.1, -58.4, -40.8, 13.8, 63.3, 38.4, 5.5, -0.1, 1.8, 24.6, 35.4, 45.4, 26.7, 15.6, 7.3, 16.3, 21.6, 11.6, 14.1, 25.5, 19.4, 4.8, -1.7, 15.9, 48.4, 26.3, 22.7, 4.0, 12.1, 5.6, -8.8, -14.9, -19.3, -17.2, -18.4, -20.7, -21.0, -8.4, -12.3, -8.0, -7.7, 12.2, 23.7, 14.7, -2.3, -15.4, -12.5, -3.7, 4.6, 8.3, 0.4, -0.4, -3.3, 0.0, -8.1],
    [1.6, -4.2, -11.3, -15.6, -6.9, 7.2, 20.7, 22.8, 15.5, 8.1, 8.1, 17.1, 20.3, 17.8, 10.6, 12.1, 18.2, 12.7, 8.0, -5.4, -6.0, -2.5, -4.2, -0.1, 3.2, 15.0, 21.0, 10.3, -6.6, -18.1, -27.5, -15.2, -15.5, -4.1, -2.8, 10.1, 18.7, 11.0, 0.7, -5.8, -10.3, -6.6, -5.4, -0.9, -0.1, -3.1, 1.5, 1.2, 3.6, -1.0, -0.9, 8.3, 16.5, 9.0, -3.3, -11.3, -4.7],
    [8.8, 0.7, -4.5, -8.8, -5.6, 0.3, 4.2, 6.7, 7.7, 10.8, 14.1, 12.8, 16.4, 12.1, 7.4, 4.2, 9.4, 7.0, 2.0, -3.7, -2.5, -0.3, 0.0, 2.1, 5.5, 11.1, 23.7, 18.8, 12.1, -4.3, -13.2, -14.1, -9.7, -0.4, 0.2, -1.3, -1.6, -0.5, -1.5, 0.7, -3.1, -3.9, -5.4, -4.1, 1.6, -1.1, 1.6, -3.6, -3.4, -5.5, -2.0, -1.5, 1.0, -2.1, -2.4, -5.8, -0.3]
]

data = np.array(values)

# Plot
fig, ax = plt.subplots(figsize=(14, 6))
fig.subplots_adjust(bottom=0.25)

# Determine symmetric range around zero
max_abs = np.max(np.abs(data))
im = ax.imshow(data, cmap='RdYlBu_r', aspect='auto', vmin=-max_abs, vmax=max_abs)

# Axis ticks and labels
ax.set_xticks(np.arange(len(dates)))
ax.set_xticklabels(dates, rotation=90, fontsize=8)
ax.set_yticks(np.arange(len(commodities)))
ax.set_yticklabels(commodities, fontsize=12)

# Labels and title
ax.set_xlabel('Month', fontsize=14)
ax.set_title('Monthly Commodity Price Change (%)', fontsize=16, fontweight='bold')

# Gridlines
ax.set_xticks(np.arange(data.shape[1] + 1) - 0.5, minor=True)
ax.set_yticks(np.arange(data.shape[0] + 1) - 0.5, minor=True)
ax.grid(which='minor', color='white', linestyle='-', linewidth=2)
ax.tick_params(which='minor', bottom=False, left=False)

# Colorbar
cbar = fig.colorbar(im, ax=ax, orientation='horizontal', pad=0.3, aspect=40, shrink=0.8)
cbar.set_label('Change (%)', fontsize=12)
cbar.ax.tick_params(labelsize=12)

plt.show()

==> figures/src/code/color.tex <==
\begin{wideexample}{Color evaluation code}\tiny

\lstinputlisting[
  language=Python,
  firstline=1,      % 想分段时随时改行号
  % lastline=100,   % 例如先显示前 100 行
]{figures/src/eval_code/color.tex}

\end{wideexample}

==> figures/src/eval_code/code.tex <==
% # code_evaluator.py (V10.8 - Final Version with Time Tracking)
% import os
% import sys
% import json
% import logging
% import argparse
% from pathlib import Path
% from typing import Dict, Any, Optional, Tuple, List
% from concurrent.futures import ProcessPoolExecutor, TimeoutError, as_completed
% from datetime import datetime
% from collections import Counter
% import io
% from contextlib import redirect_stdout
% import runpy
% import multiprocessing
% from enum import Enum
% import time # --- ADDED: Import the time module ---

% from dotenv import load_dotenv

% import matplotlib
% matplotlib.use('Agg')
% import matplotlib.pyplot as plt

% # --- Import all V9+ versioned individual evaluators ---
% try:
%     from color_evaluator import ColorEvaluator, ColorMetrics, ExecutionStatus
%     from grid_evaluator import GridEvaluator, GridMetrics
%     from layout_evaluator import LayoutEvaluator, LayoutMetrics
%     from legend_evaluator import LegendEvaluator, LegendMetrics
%     from parameter_evaluator import ParameterEvaluator, ParameterMetrics
%     from text_evaluator import TextEvaluator, TextMetrics
%     from type_evaluator import ChartTypeEvaluator, ChartTypeMetrics
% except ImportError as e:
%     print(f"Failed to import a sub-evaluator: {e}")
%     print("Please ensure all V9+ versioned evaluator .py files are present and correct.")
%     sys.exit(1)

% # --- Core Configuration ---
% logging.basicConfig(level=logging.INFO, format='%(asctime)s - %(message)s')
% logger = logging.getLogger("CodeEvaluator")
% load_dotenv()
% PROJECT_PATH = Path(os.environ.get("PROJECT_PATH", Path(__file__).parent.resolve()))

% # --- V10.6: Final Robust Code Executor ---
% def _execute_code_runner(code_file_path: str) -> Tuple[bool, Optional[str]]:
%     import runpy, matplotlib, io, os
%     from contextlib import redirect_stdout
%     matplotlib.use('Agg')
%     import matplotlib.pyplot as plt
%     plt.show = plt.savefig = lambda *args, **kwargs: None
%     plt.close('all')
%     output_buffer = io.StringIO()
%     script_path = Path(code_file_path)
%     original_directory = os.getcwd()
%     try:
%         os.chdir(script_path.parent)
%         with redirect_stdout(output_buffer):
%             runpy.run_path(script_path.name, run_name='__main__')
%         return True, None
%     except Exception as e:
%         return False, f"Error during code execution: {e}"
%     finally:
%         os.chdir(original_directory)
%         plt.close('all')

% def execute_code_and_get_figure(code_file_path: str, timeout: int = 60) -> Tuple[Optional[plt.Figure], Optional[str]]:
%     with ProcessPoolExecutor(max_workers=1) as executor:
%         future = executor.submit(_execute_code_runner, code_file_path)
%         try:
%             success, error_msg = future.result(timeout=timeout)
%             if not success: return None, error_msg
%         except TimeoutError:
%             return None, f"Code execution timed out (> {timeout} seconds)"
%         except Exception as e:
%             return None, f"Executor encountered an unknown error: {e}"

%     plt.close('all')
%     original_show = plt.show
%     original_savefig = plt.savefig
%     plt.show = lambda *args, **kwargs: None
%     plt.savefig = lambda *args, **kwargs: None
%     output_buffer = io.StringIO()
%     script_path = Path(code_file_path)
%     original_directory = os.getcwd()
%     try:
%         os.chdir(script_path.parent)
%         with redirect_stdout(output_buffer):
%             runpy.run_path(script_path.name, run_name='__main__')
%         fig_nums = plt.get_fignums()
%         if not fig_nums: return None, "Code executed successfully but did not generate any Figure"
%         return plt.figure(fig_nums[-1]), None
%     except Exception as e:
%         return None, f"Error while capturing Figure object: {e}"
%     finally:
%         plt.show = original_show
%         plt.savefig = original_savefig
%         os.chdir(original_directory)
%         plt.close('all')

% # --- Helper function for JSON serialization ---
% def convert_metrics_to_dict(metrics: Any) -> Dict[str, Any]:
%     if not isinstance(metrics, object) or not hasattr(metrics, '__dict__'):
%         return metrics
%     result_dict = {}
%     for key, value in metrics.__dict__.items():
%         if isinstance(value, Enum):
%             result_dict[key] = value.value
%         elif hasattr(value, '__dict__'):
%             result_dict[key] = convert_metrics_to_dict(value)
%         else:
%             result_dict[key] = value
%     return result_dict

% # --- Parallel Worker Function ---
% def evaluate_and_save_single_file(
%     file_name: str, 
%     generation_dir: str, 
%     gt_dir: str, 
%     results_dir: str
% ) -> Tuple[str, Dict[str, Any]]:
%     logger.info(f"Processing: {file_name}...")
%     generation_file_path = str(Path(generation_dir) / file_name)
%     gt_file_path = str(Path(gt_dir) / file_name)
%     gen_fig, gen_err = execute_code_and_get_figure(generation_file_path)
%     gt_fig, gt_err = execute_code_and_get_figure(gt_file_path)
%     full_report = {}
%     EXECUTION_SUCCESS = not (gen_err or gt_err)
%     execution_error_msg = f"GenErr: {gen_err}; GtErr: {gt_err}"
    
%     def run_evaluation(dim_name, evaluator_class, *args):
%         evaluator_instance = evaluator_class()
%         if EXECUTION_SUCCESS:
%             metrics = evaluator_instance(*args)
%             return convert_metrics_to_dict(metrics)
%         else:
%             metrics_class = globals()[evaluator_class.__name__.replace("Evaluator", "Metrics")]
%             return convert_metrics_to_dict(metrics_class(status=ExecutionStatus.FAILED, error_message=execution_error_msg))

%     full_report['color'] = run_evaluation('color', ColorEvaluator, gen_fig, gt_fig)
%     full_report['layout'] = run_evaluation('layout', LayoutEvaluator, gen_fig, gt_fig, generation_file_path, gt_file_path)
%     full_report['grid'] = run_evaluation('grid', GridEvaluator, gen_fig, gt_fig)
%     full_report['legend'] = run_evaluation('legend', LegendEvaluator, gen_fig, gt_fig)
%     full_report['parameter'] = run_evaluation('parameter', ParameterEvaluator, gen_fig, gt_fig)
%     full_report['text'] = run_evaluation('text', TextEvaluator, gen_fig, gt_fig)
%     full_report['type'] = run_evaluation('type', ChartTypeEvaluator, gen_fig, gt_fig)
    
%     output_path = Path(results_dir) / f"{Path(file_name).stem}_report.json"
%     with open(output_path, 'w', encoding='utf-8') as f:
%         json.dump(full_report, f, indent=2, ensure_ascii=False)
        
%     summary_data = {'file_name': file_name, 'is_success': EXECUTION_SUCCESS}
%     if not EXECUTION_SUCCESS:
%         summary_data['error_message'] = execution_error_msg
        
%     for dim, result in full_report.items():
%         if result.get('status') == 'success':
%             if dim == 'parameter':
%                  summary_data[f'{dim}_data_f1'] = result.get('data_metrics', {}).get('f1', 0)
%                  summary_data[f'{dim}_visual_f1'] = result.get('visual_metrics', {}).get('f1', 0)
%             else:
%                 summary_data[f'{dim}_f1'] = result.get('f1', 0)
    
%     logger.info(f"Finished: {file_name} {'(Success)' if EXECUTION_SUCCESS else '(Failed)'}")
%     return file_name, summary_data

# --- Main Evaluator Class ---
class CodeEvaluator:
    def evaluate_and_report(self, generation_dir: str, gt_dir: str, num_workers: Optional[int] = None):
        gen_path = Path(generation_dir)
        gt_path = Path(gt_dir)
        gen_files = {f.name for f in gen_path.glob("*.py")}
        gt_files = {f.name for f in gt_path.glob("*.py")}
        common_files = sorted(list(gen_files & gt_files))
        
        if not common_files:
            logger.warning("No matching Python (.py) file pairs found"); return
        if num_workers is None: num_workers = os.cpu_count()
        
        timestamp = datetime.now().strftime('%Y%m%d_%H%M%S')
        individual_results_dir = gen_path / f"_base_evaluation_{timestamp}"
        summary_report_path = gen_path / f"_metric_report_{timestamp}.json"
        error_log_path = gen_path / f"_error_log_{timestamp}.json"
        individual_results_dir.mkdir(parents=True, exist_ok=True)

        logger.info(f"Found {len(common_files)} file pairs. Using {num_workers} workers.")
        logger.info(f"Individual reports will be saved in: {individual_results_dir}")
        logger.info(f"Final summary report will be saved in: {summary_report_path}")
        logger.info(f"Error log for failed files will be saved in: {error_log_path}")

        all_summaries = []
        with ProcessPoolExecutor(max_workers=num_workers) as executor:
            future_to_file = {
                executor.submit(evaluate_and_save_single_file, fname, generation_dir, gt_dir, str(individual_results_dir)): fname 
                for fname in common_files
            }
            for future in as_completed(future_to_file):
                file_name = future_to_file[future]
                try:
                    _, summary_data = future.result()
                    all_summaries.append(summary_data)
                except Exception as e:
                    logger.error(f"Critical error for {file_name}: {e}", exc_info=True)
                    all_summaries.append({'file_name': file_name, 'is_success': False, 'error_message': str(e)})

        self._generate_summary_report(all_summaries, str(summary_report_path), str(error_log_path), generation_dir, gt_dir)

    def _generate_summary_report(self, all_summaries: List[Dict], output_path: str, error_log_path: str, gen_dir: str, gt_dir: str):
        if not all_summaries:
            logger.warning("No summary data to generate report."); return

        successful_summaries = [s for s in all_summaries if s.get('is_success')]
        failed_summaries = [s for s in all_summaries if not s.get('is_success')]
        avg_scores = Counter()
        counts = Counter()
        for summary in successful_summaries:
            for key, value in summary.items():
                if key.endswith('_f1'):
                    avg_scores[key] += value if isinstance(value, (int, float)) else 0
                    counts[key] += 1
        for key in avg_scores:
            if counts[key] > 0:
                avg_scores[key] /= counts[key]
        
        total_files = len(all_summaries)
        success_count = len(successful_summaries)
        
        report = {
            "evaluation_info": { "timestamp": datetime.now().isoformat(), "generation_directory": gen_dir, "gt_directory": gt_dir, "total_files_evaluated": total_files },
            "success_rate": { "count": success_count, "total": total_files, "rate": round(success_count / total_files, 4) if total_files > 0 else 0 },
            "average_f1_scores_on_success": {k: round(v, 4) for k, v in sorted(avg_scores.items())}
        }
        with open(output_path, 'w', encoding='utf-8') as f:
            json.dump(report, f, indent=2, ensure_ascii=False)
        logger.info(f"Comprehensive summary report saved to: {output_path}")







==> figures/src/eval_code/color.tex <==
class ColorEvaluator:
    TYPE_WEIGHTS = {
        'patch_face': 1.0,         
        'line_color': 1.0,        
        'scatter_color': 1.0,      
        'scatter_palette': 0.7,    
        'text_color': 1.0,         
        'poly3d_palette': 0.7,     
        'patch_edge': 0.01,
        'axes_bg': 0.01,
        'figure_bg': 0.01,
        'spine': 0.01,
        'tick_label': 0.05,
        'axis_label': 0.05,
        'title': 0.05,
        'legend_text': 0.05,
        'legend_bg': 0.01,
    }
    DEFAULT_WEIGHT = 0.1

    def __init__(self) -> None:
        self.metrics = ColorMetrics()

    def __call__(self, gen_fig: Optional[Figure], gt_fig: Optional[Figure]) -> ColorMetrics:
        if gen_fig is None or gt_fig is None:
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = "can not find Figure "
            return self.metrics
        try:
            generation_data = self._extract_colors_from_figure_expert(gen_fig)
            gt_data = self._extract_colors_from_figure_expert(gt_fig)
            self._calculate_metrics(generation_data, gt_data)
        except Exception as e:
            logger.error(f"color evaluate error: {e}", exc_info=True)
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = str(e)
        return self.metrics

    def _extract_colors_from_figure_expert(self, figure: Figure) -> Dict[str, Dict[str, str]]:

        extracted_data = defaultdict(dict)
        fallback_counters = defaultdict(int)

        if color := convert_color_to_hex(figure.patch.get_facecolor()): extracted_data['figure_bg']['figure'] = color

        for ax in figure.axes:
            if color := convert_color_to_hex(ax.patch.get_facecolor()): extracted_data['axes_bg'][f'ax_{id(ax)}'] = color

            if ax.get_legend():
                for handle, label in zip(ax.get_legend().legend_handles, ax.get_legend().get_texts()):
                    key = label.get_text()
                    color = None
                    if hasattr(handle, 'get_facecolor'): color = convert_color_to_hex(handle.get_facecolor())
                    elif hasattr(handle, 'get_color'): color = convert_color_to_hex(handle.get_color())
                    if color:
                        if isinstance(handle, plt.Rectangle): extracted_data['patch_face'][key] = color
                        else: extracted_data['line_color'][key] = color

            try:
                tick_labels = [tick.get_text() for tick in ax.get_xticklabels()]
                for i, patch in enumerate(ax.patches):
                    if color := convert_color_to_hex(patch.get_facecolor()):
                        key = tick_labels[i] if i < len(tick_labels) and tick_labels[i] else None
                        if not key: key = f"patch_{fallback_counters['patch_face']}"; fallback_counters['patch_face'] += 1
                        if key not in extracted_data['patch_face']: extracted_data['patch_face'][key] = color
                    if e_color := convert_color_to_hex(patch.get_edgecolor()):
                        key = tick_labels[i] if i < len(tick_labels) and tick_labels[i] else f"patch_edge_{i}"
                        extracted_data['patch_edge'][key] = e_color
            except Exception as e: logger.warning(f"handing Patches error: {e}")


            try:
                for line in ax.lines:
                    if color := convert_color_to_hex(line.get_color()):
                        key = line.get_label()
                        if not key or key.startswith('_'): key = f"line_{fallback_counters['line_color']}"; fallback_counters['line_color'] += 1
                        if key not in extracted_data['line_color']: extracted_data['line_color'][key] = color
            except Exception as e: logger.warning(f"handing Lines error: {e}")

            try:
                for collection in ax.collections:
                    colors = collection.get_facecolors()
                    if len(colors) == 0: continue

                    if len(set(map(tuple, colors))) == 1:
                        if color := convert_color_to_hex(colors[0]):
                            key = collection.get_label()
                            if not key or key.startswith('_'): key = f"scatter_group_{fallback_counters['scatter_color']}"; fallback_counters['scatter_color'] += 1
                            if key not in extracted_data['scatter_color']: extracted_data['scatter_color'][key] = color

                    else:
                        for c in {convert_color_to_hex(c) for c in colors if c is not None}:
                            key = f"palette_color_{fallback_counters['scatter_palette']}"; fallback_counters['scatter_palette'] += 1
                            extracted_data['scatter_palette'][key] = c
            except Exception as e: logger.warning(f"handle Collections error: {e}")


            try:
                for text in ax.texts:
                    if color := convert_color_to_hex(text.get_color()):
                        key = text.get_text()
                        if key: extracted_data['text_color'][key] = color
            except Exception as e: logger.warning(f"handle Texts error: {e}")
            

            if (color := convert_color_to_hex(ax.title.get_color())): extracted_data['title']['title'] = color
            if (color := convert_color_to_hex(ax.xaxis.label.get_color())): extracted_data['axis_label']['xlabel'] = color
            if (color := convert_color_to_hex(ax.yaxis.label.get_color())): extracted_data['axis_label']['ylabel'] = color

        return dict(extracted_data)


==> figures/src/eval_code/data.tex <==

# --- V10: Hardened Evaluator Class with Strict Logic ---
class ParameterEvaluator:
    def __init__(self) -> None:
        self.metrics = ParameterMetrics()
        self.DATA_PARAM_KEYS = {'xdata', 'ydata', 'offsets', 'xy', 'verts', 'width', 'height', 'sizes'}
        self.IGNORED_PARAMS = {'color', 'c', 'colors', 'label', 'labels', 'edgecolor', 'facecolor'}

    def __call__(self, gen_fig: Optional[plt.Figure], gt_fig: Optional[plt.Figure]) -> ParameterMetrics:
        if gen_fig is None or gt_fig is None:
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = "Could not get a valid Figure object"
            return self.metrics
        try:
            gen_params = self._extract_params_from_figure(gen_fig)
            gt_params = self._extract_params_from_figure(gt_fig)
            self._calculate_strict_metrics(gen_params, gt_params)
        except Exception as e:
            logger.error(f"Error during parameter evaluation: {e}", exc_info=True)
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = str(e)
        return self.metrics

    def _extract_params_from_figure(self, fig: plt.Figure) -> List[Dict]:
        extracted_params = []
        for ax in fig.axes:
            for line in ax.lines:
                params = {
                    'type': 'line', 'xdata': np.array(line.get_xdata()).tolist(), 'ydata': np.array(line.get_ydata()).tolist(),
                    'linestyle': line.get_linestyle(), 'linewidth': line.get_linewidth(), 'marker': line.get_marker(),
                    'markersize': line.get_markersize(), 'alpha': line.get_alpha()
                }
                extracted_params.append(params)

            # --- HERE IS THE FIX ---
            # Differentiate between different types of patches
            for patch in ax.patches:
                params = {'alpha': patch.get_alpha()}
                # If it's a Rectangle (from bar, hist), get width and height
                if isinstance(patch, Rectangle):
                    params.update({
                        'type': 'rectangle_patch',
                        'xy': np.array(patch.get_xy()).tolist(),
                        'width': patch.get_width(),
                        'height': patch.get_height(),
                    })
                    extracted_params.append(params)
                # If it's a Polygon (from fill, violinplot), get vertices
                elif isinstance(patch, Polygon):
                    params.update({
                        'type': 'polygon_patch',
                        'verts': np.array(patch.get_xy()).tolist(),
                    })
                    extracted_params.append(params)
                # Can add more patch types here (e.g., Circle, Ellipse) if needed
            
            for collection in ax.collections:
                params = {'type': 'collection', 'alpha': collection.get_alpha()}
                if hasattr(collection, 'get_offsets'):
                    params['offsets'] = np.array(collection.get_offsets()).tolist()
                if hasattr(collection, 'get_sizes'):
                    params['sizes'] = np.array(collection.get_sizes()).tolist()
                if len(params) > 2: # Check if any data was actually added besides type and alpha
                    extracted_params.append(params)
        return extracted_params

    def _calculate_value_similarity(self, val1: Any, val2: Any) -> float:
        """Strictly compares two values, handling numerics, strings, and lists/arrays."""
        if val1 is None and val2 is None: return 1.0
        if val1 is None or val2 is None: return 0.0
        try:
            if isinstance(val1, str): val1 = float(val1)
            if isinstance(val2, str): val2 = float(val2)
        except (ValueError, TypeError): pass

        if isinstance(val1, (int, float, np.number)) and isinstance(val2, (int, float, np.number)):
            return 1.0 if np.isclose(val1, val2) else 0.0
        if isinstance(val1, (bool, str)):
            return 1.0 if str(val1) == str(val2) else 0.0
        if isinstance(val1, (list, np.ndarray)):
            if not isinstance(val2, (list, np.ndarray)): return 0.0
            if not len(val1) and not len(val2): return 1.0
            if not len(val1) or not len(val2): return 0.0
            try:
                v1 = np.asarray(val1, dtype=float).flatten()
                v2 = np.asarray(val2, dtype=float).flatten()
                intersection = np.intersect1d(v1, v2).size
                union = np.union1d(v1, v2).size
                return intersection / union if union > 0 else 1.0
            except (ValueError, TypeError):
                set1, set2 = set(str(v) for v in val1), set(str(v) for v in val2)
                return len(set1.intersection(set2)) / len(set1.union(set2)) if set1.union(set2) else 1.0
        return 0.0

    def _calculate_strict_metrics(self, gen_elements: List[Dict], gt_elements: List[Dict]):
        if not gen_elements and not gt_elements:
            self.metrics.data_metrics = self.metrics.visual_metrics = ScoreBlock(1.0, 1.0, 1.0)
            return

        total_data_score, total_visual_score = 0.0, 0.0
        gt_data_count, gt_visual_count = 0, 0
        gen_data_count, gen_visual_count = 0, 0

        unmatched_gen_elements = gen_elements[:]
        for gt_elem in gt_elements:
            best_score, best_match_index = -1.0, -1
            for i, gen_elem in enumerate(unmatched_gen_elements):
                if gt_elem.get('type') == gen_elem.get('type'):
                    current_score = sum(self._calculate_value_similarity(gt_elem.get(k), gen_elem.get(k)) for k in gt_elem if k != 'type')
                    if current_score > best_score:
                        best_score, best_match_index = current_score, i
            
            if best_match_index != -1:
                matched_gen_elem = unmatched_gen_elements.pop(best_match_index)
                all_keys = set(gt_elem.keys()) | set(matched_gen_elem.keys())
                for key in all_keys:
                    if key in self.IGNORED_PARAMS or key == 'type': continue
                    category = 'data' if key in self.DATA_PARAM_KEYS else 'visual'
                    gt_val, gen_val = gt_elem.get(key), matched_gen_elem.get(key)
                    score = self._calculate_value_similarity(gt_val, gen_val)
                    if category == 'data': total_data_score += score
                    else: total_visual_score += score
            
            for key in gt_elem:
                if key in self.IGNORED_PARAMS or key == 'type': continue
                if key in self.DATA_PARAM_KEYS: gt_data_count += 1
                else: gt_visual_count += 1
        
        for gen_elem in gen_elements:
             for key in gen_elem:
                if key in self.IGNORED_PARAMS or key == 'type': continue
                if key in self.DATA_PARAM_KEYS: gen_data_count += 1
                else: gen_visual_count += 1

        data_p = total_data_score / gen_data_count if gen_data_count > 0 else 1.0 if not gt_data_count else 0.0
        data_r = total_data_score / gt_data_count if gt_data_count > 0 else 1.0 if not gen_data_count else 0.0
        data_f1 = 2 * (data_p * data_r) / (data_p + data_r) if (data_p + data_r) > 0 else 0.0
        self.metrics.data_metrics = ScoreBlock(data_p, data_r, data_f1)
        
        visual_p = total_visual_score / gen_visual_count if gen_visual_count > 0 else 1.0 if not gt_visual_count else 0.0
        visual_r = total_visual_score / gt_visual_count if gt_visual_count > 0 else 1.0 if not gen_visual_count else 0.0
        visual_f1 = 2 * (visual_p * visual_r) / (visual_p + visual_r) if (visual_p + visual_r) > 0 else 0.0
        self.metrics.visual_metrics = ScoreBlock(visual_p, visual_r, visual_f1)

==> figures/src/eval_code/visual.tex <==
class ParameterEvaluator:
    def __init__(self) -> None:
        self.metrics = ParameterMetrics()
        self.DATA_PARAM_KEYS = {'xdata', 'ydata', 'offsets', 'xy', 'verts', 'width', 'height', 'sizes'}
        self.IGNORED_PARAMS = {'color', 'c', 'colors', 'label', 'labels', 'edgecolor', 'facecolor'}

    def __call__(self, gen_fig: Optional[plt.Figure], gt_fig: Optional[plt.Figure]) -> ParameterMetrics:
        if gen_fig is None or gt_fig is None:
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = "Could not get a valid Figure object"
            return self.metrics
        try:
            gen_params = self._extract_params_from_figure(gen_fig)
            gt_params = self._extract_params_from_figure(gt_fig)
            self._calculate_strict_metrics(gen_params, gt_params)
        except Exception as e:
            logger.error(f"Error during parameter evaluation: {e}", exc_info=True)
            self.metrics.status = ExecutionStatus.FAILED
            self.metrics.error_message = str(e)
        return self.metrics

    def _extract_params_from_figure(self, fig: plt.Figure) -> List[Dict]:
       
        extracted_params = []
        for ax in fig.axes:
            for line in ax.lines:
                params = {
                    'type': 'line', 'xdata': np.array(line.get_xdata()).tolist(), 'ydata': np.array(line.get_ydata()).tolist(),
                    'linestyle': line.get_linestyle(), 'linewidth': line.get_linewidth(), 'marker': line.get_marker(),
                    'markersize': line.get_markersize(), 'alpha': line.get_alpha()
                }
                extracted_params.append(params)

            for patch in ax.patches:
                params = {'alpha': patch.get_alpha()}
                if isinstance(patch, Rectangle):
                    params.update({
                        'type': 'rectangle_patch',
                        'xy': np.array(patch.get_xy()).tolist(),
                        'width': patch.get_width(),
                        'height': patch.get_height(),
                    })
                    extracted_params.append(params)
                elif isinstance(patch, Polygon):
                    params.update({
                        'type': 'polygon_patch',
                        'verts': np.array(patch.get_xy()).tolist(),
                    })
                    extracted_params.append(params)
            
            for collection in ax.collections:
                params = {'type': 'collection', 'alpha': collection.get_alpha()}
                if hasattr(collection, 'get_offsets'):
                    params['offsets'] = np.array(collection.get_offsets()).tolist()
                if hasattr(collection, 'get_sizes'):
                    params['sizes'] = np.array(collection.get_sizes()).tolist()
                if len(params) > 2:
                    extracted_params.append(params)
        return extracted_params

    def _calculate_value_similarity(self, val1: Any, val2: Any) -> float:
        if val1 is None and val2 is None: return 1.0
        if val1 is None or val2 is None: return 0.0
        try:
            if isinstance(val1, str): val1 = float(val1)
            if isinstance(val2, str): val2 = float(val2)
        except (ValueError, TypeError): pass

        if isinstance(val1, (int, float, np.number)) and isinstance(val2, (int, float, np.number)):
            return 1.0 if np.isclose(val1, val2) else 0.0
        if isinstance(val1, (bool, str)):
            return 1.0 if str(val1) == str(val2) else 0.0
        if isinstance(val1, (list, np.ndarray)):
            if not isinstance(val2, (list, np.ndarray)): return 0.0
            if not len(val1) and not len(val2): return 1.0
            if not len(val1) or not len(val2): return 0.0
            try:
                v1 = np.asarray(val1, dtype=float).flatten()
                v2 = np.asarray(val2, dtype=float).flatten()
                intersection = np.intersect1d(v1, v2).size
                union = np.union1d(v1, v2).size
                return intersection / union if union > 0 else 1.0
            except (ValueError, TypeError):
                set1, set2 = set(str(v) for v in val1), set(str(v) for v in val2)
                return len(set1.intersection(set2)) / len(set1.union(set2)) if set1.union(set2) else 1.0
        return 0.0

    def _calculate_strict_metrics(self, gen_elements: List[Dict], gt_elements: List[Dict]):
        
        if not gen_elements and not gt_elements:
            self.metrics.data_metrics = self.metrics.visual_metrics = ScoreBlock(1.0, 1.0, 1.0)
            return

        total_data_score, total_visual_score = 0.0, 0.0
        gt_data_count, gt_visual_count = 0, 0
        gen_data_count, gen_visual_count = 0, 0

        unmatched_gen_elements = gen_elements[:]
        for gt_elem in gt_elements:
            best_score, best_match_index = -1.0, -1
            for i, gen_elem in enumerate(unmatched_gen_elements):
                if gt_elem.get('type') == gen_elem.get('type'):
                    current_score = sum(self._calculate_value_similarity(gt_elem.get(k), gen_elem.get(k)) for k in gt_elem if k != 'type')
                    if current_score > best_score:
                        best_score, best_match_index = current_score, i
            
            if best_match_index != -1:
                matched_gen_elem = unmatched_gen_elements.pop(best_match_index)
                all_keys = set(gt_elem.keys()) | set(matched_gen_elem.keys())
                for key in all_keys:
                    if key in self.IGNORED_PARAMS or key == 'type': continue
                    category = 'data' if key in self.DATA_PARAM_KEYS else 'visual'
                    gt_val, gen_val = gt_elem.get(key), matched_gen_elem.get(key)
                    score = self._calculate_value_similarity(gt_val, gen_val)
                    if category == 'data': total_data_score += score
                    else: total_visual_score += score
            
            for key in gt_elem:
                if key in self.IGNORED_PARAMS or key == 'type': continue
                if key in self.DATA_PARAM_KEYS: gt_data_count += 1
                else: gt_visual_count += 1
        
        for gen_elem in gen_elements:
             for key in gen_elem:
                if key in self.IGNORED_PARAMS or key == 'type': continue
                if key in self.DATA_PARAM_KEYS: gen_data_count += 1
                else: gen_visual_count += 1

        data_p = total_data_score / gen_data_count if gen_data_count > 0 else 1.0 if not gt_data_count else 0.0
        data_r = total_data_score / gt_data_count if gt_data_count > 0 else 1.0 if not gen_data_count else 0.0
        data_f1 = 2 * (data_p * data_r) / (data_p + data_r) if (data_p + data_r) > 0 else 0.0
        self.metrics.data_metrics = ScoreBlock(data_p, data_r, data_f1)
        
        visual_p = total_visual_score / gen_visual_count if gen_visual_count > 0 else 1.0 if not gt_visual_count else 0.0
        visual_r = total_visual_score / gt_visual_count if gt_visual_count > 0 else 1.0 if not gen_visual_count else 0.0
        visual_f1 = 2 * (visual_p * visual_r) / (visual_p + visual_r) if (visual_p + visual_r) > 0 else 0.0
        self.metrics.visual_metrics = ScoreBlock(visual_p, visual_r, visual_f1)
